Towards Robotic Operation with the First G-APD Cherenkov Telescope

The First G-APD Cherenkov Telecope is an Imaging Air Cherenkov Tele- scope operating since 2011 at the Observatorio del Roque de los Muchachos. One of the major goals of the FACT collaboration is to achieve robotic operation of the telescope. Since 2011 FACT is operated remotely. To reduce the necessity of human interven- tion, several programs were developed, most notably the shifthelper together with the pycustos library. This software monitors the telescope system and environmental conditions and calls the shifters in case human intervention is required. This will lead to FACT being the first IACT with all shifters asleep during regular observations. The software presented here is open source and under MIT License.

==> affil_list.tex <==
\affil{$^1$Institution Name, Institution City, State/Province, Country; \email{AuthorEmail@email.edu}}
\affil{$^2$Institution Name, Institution City, State/Province, Country}
\affil{$^3$Institution Name, Institution City, State/Province, Country}


==> author_list.tex <==
Sample~Author1,$^1$
Sample~Author2,$^2$
and
Sample~Author3$^3$

